Misspecification of Multiple Scattering in Scalar Wave Fields and its Impact in Ultrasound Tomography

In this work, we investigate the localization of targets in the presence of multiple scattering. We focus on the often omitted scenario in which measurement data is affected by multiple scattering, and a simpler model is employed in the estimation. We study the impact of such model mismatch by means of the Misspecified Cram\'er-Rao Bound (MCRB). In numerical simulations inspired by tomographic inspection in ultrasound nondestructive testing, the MCRB is shown to correctly describe the estimation variance of localization parameters under misspecification of the wave propagation model. We provide extensive discussion on the utility of the MCRB in the practical task of verifying whether a chosen misspecified model is suitable for localization based on the properties of the maximum likelihood estimator and the nuanced distinction between bias and parameter space differences. Finally, we highlight that careful interpretation is needed whenever employing the classical CRB in the presence of mismatch through numerical examples based on the Born approximation and other simplified propagation models stemming from it.

==> TikZ_sketches/AVLK.tex <==
\begin{tikzpicture}[%
    >=triangle 60,              % Nice arrows; your taste may be different
    start chain=going below,    % General flow is top-to-bottom
    node distance=6mm and 60mm, % Global setup of box spacing
    every join/.style={norm}    % Default linetype for connecting boxes
    ]

\tikzset{
  base/.style={draw, on chain, on grid, align=center, minimum height=4ex},
  sharp/.style={base, rectangle, text width=16em},
  cond/.style={base, diamond, aspect=2, text width=5em},
  rounded/.style={sharp, rounded corners},
  % coord node style is used for placing corners of connecting lines
  coord/.style={coordinate, on chain, on grid, node distance=6mm and 25mm},
  % nmark node style is used for coordinate debugging marks
  nmark/.style={draw, cyan, circle, font={\sffamily\bfseries}},
  norm/.style={->, draw},
  it/.style={font={\small\itshape}}
}

\node[sharp] (p0) {Initialize AVLK with $\finc$ and $\bm{\gamma}$};
\node[rounded, densely dotted, join] (p1) {Compute $\ftot$ using $\bm{\gamma}$. This is only an intermediate quantity.};
\node[sharp, join] (p2) {Compute $\fsc$ using $\bm{\gamma}$ and $\ftot$};
\end{tikzpicture}

==> sections/open_questions.tex <==
\subsection{open questions}

\red{The questions are still open for subsection \ref{subsec_missp}:}
\begin{itemize}
	\item \red{existence of unique minimizer for Kullback-Leibler Divergence (KLD), called the Pseudo-True Solution (PTS). we can't actually show this, or at least I can't :P do we just claim it exists without proof? This is the same as saying a set of parameters exists such that our misspecified model best explains the measurement data, and no other parameter set is as good. In linear least squares, this is the same as saying the system matrix is full rank. In non-linear least squares... I don't think there's a general way of showing it.}
	\item \red{invertibility of the Hessian of the misspecified log-likelihood. We also don't show this in general but all of our experiments had an invertible Hessian.}
	\item \red{maximum likelihood estimator (MMLE), which converges almost surely to the PTS... under certain regularity conditions. We also just assume these hold. One of them includes uniqueness of the minimizer for the log likelihood.}
	\item \red{define the misspecified cramer rao bound as a function of the PTS. We can't find the PTS directly, but can find it using the MMLE based on the previous point... assuming many conditions hold (from the previous point).}
\end{itemize}

\red{How much detail do we want in subsection \ref{subsec_comp}? Is this amount ok for TUFFC or transactions in information theory?} 
 
 
